Not All Features Are Equal: Discovering Essential Features for Preserving Prediction Privacy

When receiving machine learning services from the cloud, the provider does not need to receive all features; in fact, only a subset of the features are necessary for the target prediction task. Discerning this subset is the key problem of this work. We formulate this problem as a gradient-based perturbation maximization method that discovers this subset in the input feature space with respect to the functionality of the prediction model used by the provider. After identifying the subset, our framework, Cloak, suppresses the rest of the features using utility-preserving constant values that are discovered through a separate gradient-based optimization process. We show that Cloak does not necessarily require collaboration from the service provider beyond its normal service, and can be applied in scenarios where we only have black-box access to the service provider's model. We theoretically guarantee that Cloak's optimizations reduce the upper bound of the Mutual Information (MI) between the data and the sifted representations that are sent out. Experimental results show that Cloak reduces the mutual information between the input and the sifted representations by 85.01% with only a negligible reduction in utility (1.42%). In addition, we show that Cloak greatly diminishes adversaries' ability to learn and infer non-conducive features.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations
	       

==> body/abstract.tex <==
\vspace{-5ex}
\begin{abstract}
\vspace{-1ex}
%
%Exchange of data for prediction services has become the de facto model of operation for cloud machine learning services, giving the service provider access to an unprecedented volume of data.
%
%However, this raises serious privacy concerns as the consumers lose control over all the extra information that is naturally embedded in the input.
%
%This work demonstrates that, w
When receiving machine learning based services from the cloud, the provider does not need to receive all features; in fact, only a subset of the features are necessary for the target prediction task.
%
Discerning this subset is the key problem of this work.
%
We formulate this problem as a gradient-based perturbation maximization method that discovers this subset in the input feature space with respect to the functionality of the prediction model used by the provider. 
%
After identifying the subset, our framework, \sieve, suppresses the rest of the features using utility-preserving constant values that are discovered through a separate gradient-based optimization process.
%
%These optimization processes are performed offline. During prediction, the features are accordingly suppressed and further obfuscated.
%
We show that \sieve does not necessarily require collaboration from the service provider beyond its normal service, and can be applied in scenarios where we only have black-box access to the service provider's model.
%
We theoretically guarantee that \sieve's optimizations reduce the upper bound of the Mutual Information (MI) between the data and the sifted representations that are sent out.
%
Experimental results show that \sieve reduces the mutual information between the input and the sifted representations by 85.01\%  with only negligible reduction in utility (1.42\%).
%
In addition, we show that \sieve greatly diminishes adversaries' ability to learn and infer non-conducive features. 

\comment{
With consumers utilizing deep learning as a service, every day more and more personal data is sent to the cloud for prediction services.
%
Exchange of data for prediction/service has become the de facto model of operation where the service provider gains access to unprecedented volume of data, resulting in the furthermost of provider's deep learning services.
%
However, this operation raises serious privacy concerns as the consumers lose their control over all the extra information that is naturally embedded in the input.
%
This work builds upon the intuition that the provider does not need to receive all the features while only a subset of the features are conducive to the prediction task.
%
The problem becomes discerning this subset.
%
We formulate this problem as a gradient-based perturbation maximization method that discovers features in the input which are most conducive to DNN function.
%
As such, our algorithm uses a gradient-based search to sift through the features and find the conducive subset with respect to the functionality of a given pre-trained network.
%
After identifying the subset, our algorithm suppresses the rest of the features using constant values that are discovered through a separate gradient-based optimization process.
%
Our framework, dubbed \sieve, can be applied with both white-box and black-box access to the deployed DNN, by training a shadow network. 
%
These optimization processes are performed offline and during prediction, the features are accordingly suppressed and further obfuscated.
%
We theoretically show that \sieve reduces the upper bound of the Mutual Information (MI) between the data and the sifted representation that are sent out.
%
We show in our empirical experiments with four different datasets and networks that x\% of the features in the input image are excessive, and can be removed with negligible reduction in utility (xx\%) and no change to the parameters of the deployed classifiers. 
}
%
%We also demonstrate that the suppression of the non-conducive features improves privacy by preventing othe 
%
%We also show that using representations generated by \sieve, can help an already deployed classifier generate less biased decisions (post-hoc fairness). 
%

%[[[I'd cut the abstract in half.  Reviewers know they're going to read the 
%paper already, so probably don't even read it. I don't think anyone will even
%notice that it's different than the abstract in the submission system.  
%It's too detailed wordy for an abstract, anyway.]]]




















\comment{
Our framework sifts through the features and finds the most important ones, based on the amount of noise each feature can tolerate. 
%
This paper develops a gradient-based feature distinction techniques that discerns and sifts the feature space to only input the conducive subset of the features to the DNN for prediction.
%
However, consumers lose the ownership and control of their data  
%
With deep learning models being widely deployed in different contexts, more and more personal data is sent to remote servers for receiving various services.
%
Figuring out which features in the input contribute most the depoloyed DNN's decision making process and sending only those, can help preserve the privacy of users of these services.
%
\sieve, then, suppresses these features by replacing them with carefully-crafted constant values. 
%
\sieve can be applied with both white-box and black box access to the remote deployed DNN, enabling the user to protect her privacy even without any collaboration or change in infrastructure from the remote part. 
%
We theoretically show that \sieve reduces the upperbound of the Mutual Information (MI) between the data and the sifted representation. 
%
We show in our emprical experiments that x\% of the features in an image are excessive, and can be removed with negligible reduction in utility and no change to the parameters of the deployed classifiers. We also demonstrate how removing these features improves the privacy of the users. 
%
We also show that using representations generated by \sieve, can help an already deployed classifier generate less biased decisions (post-hoc fairness). 
%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%preserving the privacy of users' who send their data to get a service done Figuring out how deep learning models make their decisions and what features they rely on can help 
%
%There have been many attempts at interpreteability in the form of finding which input feature(s) or which training sample(s) have contributed to a given decision produced for a certain query.
%
%However, less effort on explaining what features contribute to the overall decision making of the dnn, and not a particular decision produced for a given input.
%
%If we know which features the DNN relies on for decision making, we could remove excessive features and protect the privacy of the users who send their data to remote parties for receiving services.
\comment{
The interpretation of deep learning models' decision making is an important and challenging issue due to their size and black-box nature. 
%
Previous attempts provide interpretability by either finding the input feature(s) or discovering the training sample(s) that affect a single decision.
%
This work, however, focuses on finding the features that collectively contribute to the overall decision making of the DNN, not a particular decision for a particular input.
%
The discovery of these features enables our framework, \sieve, to build a \textit{private}  representation of the data by removing the excessive features that do not contribute to the DNN's decision and may contain biased and private information. 
%
\sieve discovers such features through a novel gradient-based perturbation maximization method that requires no change to the parameters of the deployed classifiers.
%
\sieve, then, suppresses these features by replacing them with carefully-crafted constant values. 
%
We theoretically show that \sieve reduces the upperbound of the Mutual Information (MI) between the data and the sifted representation. 
%
In addition, our experimental results across various benchmark datasets, shows that the reduction in the MI is significant (x\%) and comes with only negligible reduction in utility (\%). 
}

\comment{
\textcolor{red}{focus on few learnable parameters so fast and scalable. finds features based on the network. }
INFerence-as-a-Service (INFaaS) in the cloud has enabled the prevalent use of Deep Neural Networks (DNNs) in home automation, targeted advertising, machine vision, etc.
%
The cloud receives the inference request as a raw input, containing a rich set of private information, that can be misused or leaked, possibly inadvertently.
%
This prevalent setting can compromise the privacy of users during the inference phase.
%
This paper sets out to provide a principled approach, dubbed \cloak, that finds optimal stochastic perturbations to obfuscate the private data before it is sent to the cloud. 
%
To this end, \cloak reduces the information content of the transmitted data while conserving the essential pieces that enable the request to be serviced accurately.
%
The key idea is formulating the discovery of this stochasticity as an \emph{offline gradient-based optimization problem} that reformulates a pre-trained DNN (with optimized known weights) as an analytical function of the stochastic perturbations.
%
Using Laplace distribution as a parametric model for the stochastic perturbations, \cloak learns the optimal parameters using \emph{gradient descent} and Monte Carlo sampling.
%
This set of optimized Laplace distributions further guarantee that the injected stochasticity satisfies the $\epsilon$-differential privacy criterion.
%
Experimental evaluations with real-world datasets show that, on average, the injected stochasticity can reduce the information content in the input data by 80.07\%, while incurring 7.12\% accuracy loss.
}

\comment{
%
The interpretation of deep learning models' decision making is an important and challenging issue due to their size and black-box nature. 
%
Previous attempts provide interpretability by either finding the input feature(s) or discovering the training sample(s) that affect a single decision.
%
This work, however, focuses on finding the features that collectively contribute to the overall decision making of the DNN, not a particular decision for a particular input.
%
The discovery of these features enables our framework, \sieve, to build a \textit{private}  representation of the data by removing the excessive features that do not contribute to the DNN's decision and may contain biased and private information. 
%
\sieve discovers such features through a novel gradient-based perturbation maximization method that requires no change to the parameters of the deployed classifiers.
%
\sieve, then, suppresses these features by replacing them with carefully-crafted constant values. 
%
We theoretically show that \sieve reduces the upperbound of the Mutual Information (MI) between the data and the sifted representation. 
%
In addition, our experimental results across various benchmark datasets, shows that the reduction in the MI is significant (x\%) and comes with only negligible reduction in utility (\%). 
}





%light-weight, no change to classifier, no need to know other private labels, latent
%
%Experimental results across various benchmark datasets show that \cloak framework offers a promising ...

%This  work, however tries to explain what feature are not important
\end{abstract}


==> body/excerpts.tex <==
\subsection{Feature-Differential Privacy}\label{sec:pixel-dp}
In the conventional differential privacy (DP) setting\cite{cynthia}, the main goal is to create an algorithm such that one cannot infer whether an individual data instance was in the dataset by observing the algorithm's output.
%making the participation of an individual 
%hiding the effect of  a single data record  within the dataset. 
In \panthomime's problem setting, however, our goal is to obfuscate personal/sensitive features, within each data instance. This problem can be looked upon as trying to make the changes in one feature within the data instance indistinguishable. For images, the features can be the pixels, and one attempt at protecting sensitive information in the image could be adding noise through a deferentially private mechanism, so as to make pixels less distinguishable. We use a feature related definition of differential privacy and call it feature differential privacy (FDP).
%which has also been used by~\cite{pixel-dp}.

\begin{defn}\textbf{$\epsilon$-FDP.} For $\epsilon\geq 0$, an algorithm $A$ satisfies $\epsilon$-FDP if and only if for any pair of datasets $D$ and $D'$ that differ in only one feature:
\begin{equation}
\mathcal{P}[A(D)=t] \leq e^\epsilon \mathcal{P}[A(D')=t]\;\;\;\forall t
\end{equation}
where, $\mathcal{P}[A(D)=t]$ denotes the probability that the algorithm $A$ outputs $t$.
In the case of image processing, the datasets $D$ and $D'$ can be two identical images that only differ in one pixel. \end{defn}

\subsection{Neural Network Partitioning}
\label{sec:NNP}
\panthomime operates by adding calibrated random perturbations to the input and creating a representation of the data that is aimed to restrict/remove the sensitive information.
%
This input data can be the raw data that is fed to the neural network, or it can be an intermediate representation, given by cutting the neural network into two sections. The latter scheme is sometimes used in edge devices~\cite{edge-partition} to off-load the compute-intensive part of the operations to a remote cloud.
%
Sending an intermediate representation instead of the raw data also helps the privacy of the users, since the abstract intermediate representation carries less information~\cite{lalitah, ali}. In this setup, $f$ denotes the function for the first part of the neural network and $g$ denotes the second part. If there is no neural network partitioning, $f$ becomes the identity function.

If \panthomime is applied in a deeper layer of the neural network, then the function $f$ is going to be the first partition of the neural network, and calculating the sensitivity becomes a complex optimization problem~\cite{pixel-dp, Lipshitz, other}. In the appendix we discuss literature on ways of acquiring an upper bound for sensitivity when \panthomime is applied to deeper layers. \fix{add to appendix.}

%%%%%%%%%%%%





During the inference phase, for each input data tensor (\tensor{D}), \cloak adds a distinct randomly generated perturbation tensor (\tensor{X}).
%
This addition yields a perturbed representation of the input that is sent out to the cloud for classification with the DNN denoted by $g$.
%
During the inference phase no optimization is performed.
%
\tensor{X} is generated by sampling each element, $x$, independently, from a Laplace distribution $Lap(\mu, b)$, where $\mu$ and $b$ are the corresponding elements of the locations (\tensor{M}) and scales tensors ( \tensor{B}).
%

In a separate \emph{offline} process, \cloak finds these \tensor{M} and \tensor{B} tensors by solving an optimization problem.
%
\panthomime trains the locations and scales tensors in such a way that: (1) provides the required differential privacy guarantee, as defined shortly; (2) incurs minimum degradation to the neural network's objective, and, (3) decreases the amount of mutual information between the original tensor \tensor{D} and its noisy, perturbed version, $A_{f}(\tensor{D})$. 
%
When the desired tensors \tensor{M} and \tensor{B} are found, they are used for perturbing input data for inference, in deployed neural networks as mentioned above.  

This section first defines an instantiation of differential privacy, called feature differential privacy, that applies to our problem setup.
%
The section continues on to discuss the constraints that need to be applied to the locations and scales tensors to meet the required guarantee and related privacy consideration. 
%
Finally, this section explain the workflow in details and provide a proof that the proposed mechanism is $\epsilon$-feature differentially private.


%%%%%%%%%%%%%%%%%%
\vspace{-1ex}
\subsection{Loss Function}
%
\label{sec:loss}
\panthomime's objective function is to minimize the mutual information (or maximize the noise variance as discussed before) subject to a bounded degradation in the neural network's utility. Using Lagrange multiplier $\lambda$ and given our reparameterization of $\tensor{B}$, we can express the loss function of \panthomime as
\begin{equation} \label{eq:loss}
   \mathcal{L}(\tensor{M},\tensor{B})= -\log{\tensor{B}} +\lambda\mathcal{L}_{nn}(\tensor{M},\tensor{B})
\end{equation}

where, $\mathcal{L}_{nn}$ represents the utility loss function of the neural network. For instance, in the case of $C$-class classification, this utility can be represented as $\mathcal{L}_{nn}(\tensor{M},\tensor{B})=-\frac{1}{n} \sum_{i=1}^{n} \sum_{c=1}^{C} y_c^i\log(p_c^i)$, which is the cross entropy loss, where $p_c^i$ is the $i^{th}$ Monte Carlo sample \cite{monte} of the probability the neural network has assigned to observation $i$ belonging to class $c$, and, $y_c^i$ is the indicator function of whether the $i^{th}$ sample belongs to the class $c$. Converting the averaging over $n$ samples into the population expectation, we can rewrite our loss function as
\begin{equation} \label{eq:loss2}
\begin{split}
    \mathcal{L}(\tensor{M},&\tensor{B})\!=\!-\log{\tensor{B}} \\&+\lambda\,\mathbb{E}_{\tensor{X}\sim L(\tensor{M},\tensor{B})}\Big[\sum_{c=1}^{C} y_c\log\left(g\big(f(\tensor{D})+\tensor{X}\big)_c\right)\Big]
    \end{split}
    \vspace{-1ex}
\end{equation}

We take sufficiently large $n$ noise samples drawn from the current locations and scales tensors to approximate the second term. This means that to apply a single update to the trainable parameters, \panthomime runs multiple forward passes on the entire neural network, at each pass draws new samples for the noise (perturbation) tensor, and averages over the losses and applies the update using the average. However, in practice, if mini-batch training is used, we observed that using only a single noise sample for each update can yield desirable results, since a new noise tensor is sampled for each mini-batch.

\vspace{-1ex}
The parameter $\lambda$ is the knob, which could be tuned to reflect whether we want to trade-off accuracy for information degradation (more privacy), or vice versa. We name the $-log\tensor{B}$, the mutual information decay term. One important feature of \cloak is that it does not need access to sensitive information/labels. In other words, it does not need to be given specific information about what it is protecting against, it only needs access to the non-sensitive labels of the main task, and it tries to remove any extra information with the trained perturbations. For more details of the optimization problem please refer to the supplementary material. 



\subsection{Average and Worst-Case Privacy Considerations} \label{sec:avg-worse}
Differential privacy offers a worst-case privacy guarantee. \cloak, however, decreases the mutual information between the input data and its perturbed representation, while maintaining the desired differential privacy guarantee. The reduction in mutual information can be considered as an average-case privacy measure~\cite{lalitha2018, lalitha17b}. 

As discussed, the mutual information between tensors \tensor{D} and $A_{f}(\tensor{D})$ where the latter is acquired by injecting noise to $f(\tensor{D})$, is proportional to the log of the standard deviation of the noise that is added to each feature (element) in $f(\tensor{D})$. Therefore, \panthomime needs to maximize the scales of the noise distributions to minimize the leaked mutual information.

Increasing the scale parameters of noise elements through training must be done in consideration of the neural network's objective. For instance, in a setting where the task is smile detection, some facial features like the mouth are conducive to this detection. Other features, however, such as that person's hair, the background, their eye color, etc. are irrelevant. Thus, adding more noise to these features can achieve higher privacy in terms of information loss, while incurring minimum degradation to the utility. 

%






An example of noise injection can be seen in Figure~\ref{fig:screen}, where the effect of increase in the average of the noise scales is illustrated for two sample images from the CelebA~\cite{celeba} dataset. 
%
In this illustration, \cloak causes non-conducive features to get blurry by increasing the scales.
%
For the rightmost images, only the smile and some  minor facial attributes are present.
%
For instance, notice the second example image where the other person in the background fades away as the noise increases. 
%
The mean accuracy drop over the test portion of the dataset for the four perturbation distribution sets (four sets of tensors \tensor{B and M}) in this Figure are 3.4\%, 3.7\%, 4.5\% and 12.7\% respectively, with standard deviations in the $0.12\%-0.68\%$ range.
%
The privacy budget ($\epsilon$) is $2.5$.

Such a rather targeted (non-uniform) obfuscation behavior that leads to low degradation in accuracy for a given $\epsilon$ is the result of our formulation that incorporates mutual information in \cloak's loss function (see Section~\ref{sec:loss}).
%
If only the differential privacy constraint was considered, the noise would have just been increased uniformly across the image and accuracy loss would have been much higher. This behavior will be discussed in more details in Section~\ref{sec:res2}.




\begin{figure*}[h]
    \centering
    \begin{subfigure}{0.6\textwidth}
     \includegraphics[width=\linewidth]{figures/colorbar.pdf}
    \end{subfigure}
    
    \begin{subfigure}{0.05\textwidth}
        \centering
        \makebox[20pt]{\raisebox{20pt}{\rotatebox[origin=c]{90}{\tiny Perturbation Intensity}}}%
    \end{subfigure}
    \begin{subfigure}{0.15\textwidth}
        \centering
        \makebox[20pt]{\raisebox{20pt}{\rotatebox[origin=c]{90}{\tiny  }}}
        %\includegraphics[width=\linewidth]{figures/heatmap-0l44.png}
         
    \end{subfigure}
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/heatmap-0l44-nobar.png}
    \end{subfigure}
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/heatmap-1l0-nobar.png}
    \end{subfigure}
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/heatmap-1l7-nobar.png}
    \end{subfigure}
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/heatmap-1l95-nobar.png}
    \end{subfigure}
    
    \begin{subfigure}{0.05\textwidth}
        \centering
        \makebox[20pt]{\raisebox{20pt}{\rotatebox[origin=c]{90}{\tiny Example 1}}}%
    \end{subfigure}
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/fig0-orig.png}
    \end{subfigure}%
    \begin{subfigure}{0.001\textwidth}
        \centering
        \makebox[20pt]{\raisebox{20pt}{\rotatebox[origin=c]{90}{\tiny  }}}
        %\includegraphics[width=\linewidth]{figures/heatmap-0l44.png}
    \end{subfigure}
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/fig0-0l44.png}
    \end{subfigure}
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/fig0-1l0.png}
    \end{subfigure}
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/fig0-1l7.png}
    \end{subfigure}
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/fig0-1l95.png}
    \end{subfigure}

    \begin{subfigure}{0.05\textwidth}
        \centering
        \makebox[20pt]{\raisebox{20pt}{\rotatebox[origin=c]{90}{\tiny Example 2}}}%
    \end{subfigure}
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/fig1-orig.png}
        \caption{Original}
    \end{subfigure}%
    \begin{subfigure}{0.001\textwidth}
        \centering
        \makebox[20pt]{\raisebox{20pt}{\rotatebox[origin=c]{90}{\tiny  }}}
        %\includegraphics[width=\linewidth]{figures/heatmap-0l44.png}
    \end{subfigure}
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/fig1-0l44.png}
        \caption{$\bar{\tensor{B}} = 0.44$}
    \end{subfigure}
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/fig1-1l0.png}
        \caption{$\bar{\tensor{B}} = 1.01 $}
    \end{subfigure}
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/fig1-1l7.png}
        \caption{$\bar{\tensor{B}} = 1.70$}
    \end{subfigure}
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/fig1-1l95.png}
        \caption{$\bar{\tensor{B}} = 1.95$}
    \end{subfigure}
    
    \caption{Visualizing the effect of \cloak on the input images as we increase the average scale of perturbations $\bar{\tensor{B}}$ that is proportional to the standard deviation. The non-sensitive classification task is smile detection. The first row shows the heat map of perturbation scales for each pixel. At higher scales, \cloak obfuscates the features that are non-conducive to the smile detection task e.g. the background, the hair, etc., while only the lips and some minor facial attributes are recognizable.}
    \label{fig:screen}
    \vspace{-1ex}
\end{figure*}


Figure~\ref{fig:sigma-suppress-compare} shows a comparison of the accuracy of these three schemes on a held-out test portion of the CelebA dataset for smile detection task. As expected, suppression with trained values has the highest accuracy, given noise maps with the same $\bar{\boldsymbol\sigma}s$. 
%
Suppression with black pixels yields the worst accuracy, especially under larger $\bar{\boldsymbol\sigma}$. This is because in cases where $\bar{\boldsymbol\sigma}$ is smaller, less features are deemed non-conducive (since most features have little noise) and therefore less features are suppressed to zero. These feauters are mostly background features that are also black in many of the images. When $\bar{\boldsymbol\sigma}$ increases, more features get higher noise and are  therefore suppressed. At this point, the non-conducive features are facial attributes as well, which the classifier is not used to them being zero, therefore accuracy drops. 
%
The noise maps for this experiment are the ones from the fourth column of Figure~\ref{fig:patterns}.


\begin{algorithm}[t]
   \caption{ Suppression-Value Training Workflow}
   \label{alg:suppress}
\begin{algorithmic}
   \STATE {\bfseries Input:} $\mathcal{D}$, $y$, $f_\theta$, $\boldsymbol\sigma$, $\boldsymbol\mu$, $mask$
    \STATE Initialize  $\boldsymbol{\mu_s}\!=\!\boldsymbol\mu$
   \REPEAT
   \STATE Select training batch $\mathbf{x}$ from $\mathcal{D}$ 
   \STATE Let $\mathbf{x} = \mathbf{x} \circ mask$
   \STATE Sample $\mathbf{e} \sim \mathcal{N}(0,1)$
   \STATE Let $\mathbf{r} = \boldsymbol{\sigma}\circ\mathbf{e} \circ mask+ \boldsymbol\mu_s$
   \STATE Take gradient step on $\boldsymbol\mu_s$ from $\mathbb{E}_{r}[\mathcal{L}_{CE}(f_{\theta}(\mathbf{x+r)},\ y)]$
   \UNTIL{Algorithm converges}
   \STATE {\bfseries Return:} $\boldsymbol\mu_s$
   
\end{algorithmic}
\end{algorithm}
\setlength{\textfloatsep}{\textfloatsepsave}


%%%%%%%%%%%%%%%%%%%

\newlength{\textfloatsepsave} \setlength{\textfloatsepsave}{\textfloatsep} \setlength{\textfloatsep}{0ex}  
\begin{algorithm}[t]
   \caption{  Perturbation Training Workflow}
   \label{alg:work}
\begin{algorithmic}
   \STATE {\bfseries Input:} $\mathcal{D}$, $y$, $f_\theta$, $m$, $\lambda$
    \STATE Initialize  $\boldsymbol{\mu}\!=\!0$, $\boldsymbol{\rho}\!=\!-10$ and $M\geq m$
   \REPEAT
   \STATE Select training batch $\mathbf{x}$ from $\mathcal{D}$ 
   \STATE Sample $\mathbf{e} \sim \mathcal{N}(0,1)$
   \STATE Let $\boldsymbol\sigma = \frac{1.0 + \tanh(\boldsymbol{\rho})}{2} (M)$
   \STATE Let $\mathbf{r} = \boldsymbol{\sigma}\circ\mathbf{e} + \boldsymbol\mu$
   \STATE Take gradient step on $\boldsymbol\mu$ and $\boldsymbol\rho$ from Equation~\eqref{eq:loss2}
   \UNTIL{Algorithm converges}
   \STATE {\bfseries Return:} $\boldsymbol\mu$, $\boldsymbol\sigma$
   
\end{algorithmic}
\end{algorithm}
\setlength{\textfloatsep}{\textfloatsepsave}


%%%%%%%%%%%%%%%%%%




%%%%%%%INTRO
%In such a consumer-based setting, the response time of the service plays a vital role in the user's experience. 
%
%The emerging adoption of always-listening home assistants and other invasive ML applications in every-day life requires measures to protect common user privacy at a high speed. 
%Cloak is intended for these everyday use cases. 
%The sent data usually contains an abundance of excessive personal  information.
%

%
%every day use cases need to be fast but can tolerate a small accuracy loss are not safty-critical edge-cloud data-learning
%The service level agreement of cloud response times is 10-100 milliseconds (based on MLPerf Industry benchmarks ~\cite{reddi2019mlperf}).

%All of the encryption-based methods have execution times of orders of magnitude higher, with communication overheads ($350\times-2850000\times$) that are unbearable for many edge devices with unstable connections. 
%

%Previous privacy preserving methods are not suitable for this setting as they either need collaboration from the service provider, significantly reduce model utility, or have prohibitive execution time. 
%%%%%%%%%

We formulate this problem as a maximization of privacy by minimizing the upper bound of the Mutual Information (MI) between the irrelevant features and the generated sifted representation, while maximizing the lower bound of MI between the relevant features and the generated representation (to preserve utility).



weights where the output of the model now is parametric with repect to the scales that are actually unkonw.

%
%
The constrain that guides the \emph{scale learning process} is that the scales should be learned in such a way that minimizes accuracy loss.
%
To this end, we formulate a loss function 

On the ones hand, we aim to maximize the scales while, one the hand, incorporation of the classification loss minimize the noise for the features that are conducive to the task.
%
This min-max optimization 



The objective is two folds: 
(a) maximize privacy by minimizing the upper bound of the Mutual Information (MI) between the irrelevant features and the generated sifted representation, (b) while maximizing the lower bound of MI between the relevant features and the generated representation (to preserve utility).
%

%
To solve the problem, we use a gradient-based process that the sifted representations are generated by Gaussian noise to each feature in the input and optimized parameters are 
%
After that, the features that can tolerate less noise are deemed conducive to the task, and features that tolerate great amounts of noise are non-conducive.   
%
\sieve then removes these non-conducive features, to protect the privacy of the consumers while maintaining the utility of the service. 




%
The goal of this optimization is to minimize the upper bound of the Mutual Information (MI) between the irrelevant features and the generated sifted representation (to maximize the privacy), while maximizing the lower bound of MI between the relevant features and the generated representation (to preserve utility). 
%
To solve the problem, we use a gradient-based process that the sifted representations are generated by Gaussian noise to each feature in the input and optimized parameters are 
%
After that, the features that can tolerate less noise are deemed conducive to the task, and features that tolerate great amounts of noise are non-conducive.   
%
\sieve then removes these non-conducive features, to protect the privacy of the consumers while maintaining the utility of the service. 
%


%%%%%%%%%%%%%


%

This paper presents \sieve, a framework that sifts the features of the data based on their relevance to the target prediction task. 
%
We formulate the discovery of relevant features as an optimization problem. 
%
The goal of this optimization is to minimize the upper bound of the Mutual Information (MI) between the irrelevant features and the generated sifted representation (to maximize the privacy), while maximizing the lower bound of MI between the relevant features and the generated representation (to preserve utility). 
%
To solve the problem, we use a gradient-based process that the sifted representations are generated by Gaussian noise to each feature in the input and optimized parameters are 
%
After that, the features that can tolerate less noise are deemed conducive to the task, and features that tolerate great amounts of noise are non-conducive.   
%
\sieve then removes these non-conducive features, to protect the privacy of the consumers while maintaining the utility of the service. 
%
By removing such features, \sieve guarantees that no information about them can be learned or inferred from the sifted representation that the consumer sends.
%

Unlike other methods~\cite{dpfe,shredder,dp,sec}, due to its execution model, the consumer can independently deploy \sieve with only black box access to the provider's model, particularly useful for scenarios where the provider is uncooperative.
%
In real world scenarios, the providers are usually reluctant to relinquish the stream of the incoming data, as it is vital for the continuation of the services since the providers usually rely on this data to improve their products and services~\cite{x,y,z}. 
%
In the black-box access scenarios, \sieve trains a substitute model that imitates the behaviour of the target predictor if fed by the data from the same distribution.
%
This substitute model then can be used for discovering the conducive features.
%
Quite similar to the substitute model that has been employed in the context of inference attacks~\cite{} as well as adversarial example attacks~\cite{}. 

\cloak offers these capabilities with a start contrast to other methods that use noise for prediction privacy that require to know what they are protecting against (i.e., a private label). 
%
\cloak, however, does not need this extra labeling and it attempts at removing any excessive information that is not conducive to the main prediction task/label.
%
While \sieve does not rely on extra labeling, it can only protect the features that do not inherently overlap with the features of the target prediction task. 
%
Additionally, unlike these techniques, \cloak does not need to know nor it does needs to change parameters or the architecture of the service provider's model.
%%%%%%%%%
\begin{wrapfigure}{r}{0.5\textwidth}
  \begin{center}
    \vspace{-4ex}
    \includegraphics[width=1\linewidth]{figures/homomorphics.pdf}
  \end{center}
  \caption{Slowdown of encryption-based methods compared to \sieve, in logarithmic scale. }
\end{wrapfigure}

We provide an analytical formulation of the problem as a constrained convex optimization program that maximizes the privacy by minimizing the mutual information between the raw input and the data sent to the cloud subject to a restriction on the degradation of the DNN utility (accuracy).
%
\cloak's objective function and the constraint both depend on the prior distribution of the perturbation.
%
However, for a fixed parameterized family of distributions and a fixed value of the Lagrange multiplier knob, the problem has a unique global optima.
%
The convexity of the formulation guarantees that the \emph{gradient descent} will converge to that global optima.
%
This proves that \cloak maximizes the privacy under the utility preserving constraint.
%

%%%%%%%%%%%%%%%%
\textcolor{red}{add if needed:}
One set of examples could be smart home devices, such as doorbell cameras that run multimedia processing or always-listening smart speakers. In medical imaging, where outsourcing the raw input is not an option, cloak provides a way forward. Zoom, used widely these days, runs inferences to detect silhouette, can be another application.

The emerging adoption of always-listening home assistants and other invasive DNNs in every-day life requires measures to protect common user privacy at a high speed. Cloak is intended for these everyday use cases. 
%%%%%%%%%%%%%

\subsection{Support for Black-Box Access Mode}

\sieve's requres access to the target model to sift features.
%
However, as shown by previous works~\cite{memberinf, shadow2},  
%
we can train a ``shadow" or ``substitute" model on similar data, and then use this model for the training of perturbations. 
%
%
This approach has been widely adopted for black-box inference attacks against machine learning models~\cite{attacks} and adversarial example attacks against deep neural networks~\cite{adv}.
%

The main challenge is  generating the training data needed for training the substitute model. 
%
Shokri et al. propose three options for this problem, in black box setting~\cite{membering}.
%
One is reverse engineering the target model and finding input data (model inversion attacks), one is using some known statistics of the data to generate similar instances, and the third one is to gain access to a potentially noisy version of the target classifier's training dataset.
%
We have taken the approach used by Shokri et al. in their experiments, which uses the third option.
%
This is a feasible option, since there is a plethora of open-access datasets for different applications.
%
%
We discuss the details of how we employ substitute models and compare their performance to white-box access in the evaluation section. 

%%%%%%%%%%%%s
